Characterisation of the Berkovich Spectrum of the Banach Algebra of Bounded Continuous Functions

For a complete valuation field k and a topological space X, we prove the universality of the underlying topological space of the Berkovich spectrum of the Banach k-algebra Cbd(X,k) of bounded continuous k-valued functions on X. This result yields three applications: a partial solution to an analogue of Kaplansky conjecture for the automatic continuity problem over a local field, comparison of two ground field extensions of Cbd(X,k), and non-Archimedean Gel'fand theory.

==> rac.tex <==
\subsection{Relation to Another Construction}
\label{Relation to Another Construction}



In the case where $k$ is a local field or a finite field, we show that $\m{BSC}_k(X)$ coincides with a space $\m{SC}_k(X)$ defined in this section. Here a {\it local field} means a complete valuation field with non-trivial discrete valuation and finite residue field.

\begin{dfn}
\label{SC}
Denote by $\m{C}_{\m{bd}}(X,k)(1) \subset \m{C}_{\m{bd}}(X,k)$ the subset $\m{C}(X,k^{\circ})$ of bounded continuous $k$-valued functions on $X$ which take values in the subring $k^{\circ} \subset k$ of integral elements, and consider the evaluation map
\begin{eqnarray*}
  \iota'_k \colon X &\to& (k^{\circ})^{\m{C}_{\m{bd}}(X,k)(1)}\\
  x &\mapsto& (f(x))_{f \in \m{C}_{\m{bd}}(X,k)(1)}.
\end{eqnarray*}
By the definition of the direct product topology, $\iota'_k$ is continuous. Denote by $\m{SC}_k(X) \subset (k^{\circ})^{\m{C}_{\m{bd}}(X,k)(1)}$ the closure of the image of $\iota'_k$. We also denote by $\iota'_k$ the continuous map $X \to \m{SC}_k(X)$ induced by $\iota'_k$.
\end{dfn}

If $k$ is a local field or a finite field, then $\m{SC}_k(X)$ is a totally disconnected compact Hausdorff space because so is $k^{\circ}$.

\begin{prp}
\label{extension property}
The space $\m{SC}_k(X)$ satisfies the following extension property: For any $f \in \m{C}_{\m{bd}}(X,k)$, there is a unique $\m{SC}_k(f) \in \m{C}_{\m{bd}}(\m{SC}_k(X),k)$ such that $f = \m{SC}_k(f) \circ \iota'_k$. Moreover, the equality $\| f \| = \| \m{SC}_k(f) \|$ holds.
\end{prp}

\begin{proof}
The uniqueness of $\m{SC}_k(f)$ and the norm-preserving property is obvious because $\iota'_k(X) \subset \m{SC}_k(X)$ is dense and $k$ is Hausdorff. We construct the extension $\m{SC}_k(f)$. Note that $|k| \subset \lbrack 0, \infty )$ is bounded if and only if $|k| = \{ 0,1 \}$. Therefore $|k| \subset \lbrack 0, \infty )$ is unbounded or closed. It implies that that there is an $a \in k^{\times}$ such that $\| f \| \leq |a|$. For an $x = (x_g)_{g \in \m{C}_{\m{bd}}(X,k)(1)} \in \m{SC}_k(X)$, the value $a x_{a^{-1}f} \in k$ is independent of the choice of an $a \in k^{\times}$, and we set $\m{SC}_k(f)(x) \coloneqq a x_{a^{-1}f}$. Indeed, let $a_1,a_2 \in k^{\times}$ and suppose $\| f \| \leq \min \{ |a_1|, |a_2| \}$. For any $y \in X$, one has $\iota'_k(y)_{a_1^{-1}f} = a_1^{-1}f(y)$ and $\iota'_k(y)_{a_2^{-1}f} = a_2^{-1}f(y)$. It implies $a_1 \iota'_k(y)_{a_1^{-1}f} = a_2 \iota'_k(y)_{a_2^{-1}f} \in k$. Since the image $\iota'_k(X) \subset \m{SC}_k(X)$ is dense, one obtains $a_1 x_{a_1^{-1}f} = a_2 x_{a_2^{-1}f} \in k$. By the discussion above, one gets $\m{SC}_k(f) \circ \iota'_k = f$. The map $\m{SC}_k(f)$ is continuous by the definition of $\m{SC}_k(X)$.
\end{proof}

\begin{crl}
\label{functoriality}
For a $(Y,\varphi) \in X/\m{Top}$, there is a unique continuous map
\begin{eqnarray*}
\begin{array}{cccc}
  \m{SC}_k(\varphi) \colon \m{SC}_k(X) \to \m{SC}_k(Y)
\end{array}
\end{eqnarray*}
such that $\m{SC}_k(\varphi) \circ \iota'_k = \iota'_k \circ \varphi$.
\end{crl}

\begin{proof}
The uniqueness of $\m{SC}_k(\varphi)$ follows from the facts that $X$ is dense in $\m{SC}_k(\varphi)$ and that $\m{SC}_k(Y)$ is Hausdorff. By Proposition \ref{extension property}, one has a unique continuous map $\m{SC}_k(\varphi) \to (k^{\circ})^{\m{C}_{\m{bd}}(X,k)(1)}$ extending the composite
\begin{eqnarray*}
\begin{array}{cccc}
  X \stackrel{\varphi}{\longrightarrow} Y \stackrel{\iota'_k}{\longrightarrow} \m{SC}_k(Y) \hookrightarrow (k^{\circ})^{\m{C}_{\m{bd}}(X,k)(1)}.
\end{array}
\end{eqnarray*}
Its image lies in the closed subspace $\m{SC}_k(Y)$ because $X$ is dense in $\m{SC}_k(X)$. One obtains a continuous map $\m{SC}_k(\varphi) \colon \m{SC}_k(X) \to \m{SC}_k(Y)$ such that $\m{SC}_k(\varphi) \circ \iota'_k = \iota'_k \circ \varphi$.
\end{proof}

Thus one has obtained a functor
\begin{eqnarray*}
\begin{array}{cccc}
  \m{SC}_k \colon & \m{Top} & \to & \m{TDCHTop} \\
  & Y & \rightsquigarrow & \m{SC}_k(Y) \\
  & (\varphi \colon Y \to Z) & \rightsquigarrow & \left( \m{SC}_k(\varphi) \colon \m{SC}_k(Y) \to \m{SC}_k(Z) \right)
\end{array}
\end{eqnarray*}
with an obvious natural transform $\iota_k \colon \m{id}_{\m{Top}} \to \m{SC}_k$. We compare $\m{BSC}_k$ with $\m{SC}_k$ in the case where $k$ is a local field or a finite field.

\begin{lmm}
\label{reflexivity 2}
Suppose that $k$ is a local field or a finite field endowed with the trivial valuation, and that $X$ is a totally disconnected compact Hausdorff space. Then $\iota'_k \colon X \to \m{SC}_k(X)$ is a homeomorphism.
\end{lmm}

\begin{proof}
By the assumption of $k$, $\m{SC}_k(X)$ is a totally disconnected compact Hausdorff space. Therefore it suffices to verify the injectivity of $\iota'_k$, because a continuous map from a compact space to a Hausdorff space is a closed map. Let $x,y \in X$ with $x \neq y$. Since $X$ is zero-dimensional and Hausdorff, there is a $U \in \m{CO}(X)$ such that $x \in U$ and $y \notin U$. Then one has $\iota'_k(x)_{1_U} = 1 \neq 0 = \iota'_k(y)_{1_U}$, and hence $\iota'_k(x) \neq \iota'_k(y)$. Thus $\iota'_k \colon X \to \m{SC}_k(X)$ is injective.
\end{proof}

\begin{prp}
\label{SC and TDC}
Suppose that $k$ is a local field or a finite field endowed with the trivial valuation. Then $\m{SC}_k(X)$ is initial in $X/\m{TDCHTop}$ with respect to $\iota'_k$.
\end{prp}

We remark that the assumption on the base field $k$ is not necessary when $X$ is compact. Analysis of continuous functions on a compact space is quite classical.

\begin{proof}
For a $(Y,\varphi) \in \m{ob}(X/\m{TDCHTop})$, we construct a continuous extension
\begin{eqnarray*}
  \psi \colon \m{SC}_k(X) \to Y
\end{eqnarray*}
of $\varphi$ in an explicit way. An extension $\psi$ is unique if it exists, because the image of $X$ is dense in $\m{SC}_k(X)$ and $Y$ is Hausdorff. Consider the commutative diagram
\begin{eqnarray*}
\begin{CD}
  X           @>{\varphi}>>           Y \\
  @V{\iota'_k}VV                      @VV{\iota'_k}V \\
  \m{SC}_k(X) @>>{\m{SC}_k(\varphi)}> \m{SC}_k(Y)
\end{CD}.
\end{eqnarray*}
By Lemma \ref{reflexivity 2}, the right vertical map is a homeomorphism, and one obtains a continuous map $\psi \coloneqq \iota'_k{}^{-1} \circ \m{SC}_k(\varphi) \colon \m{SC}_k(X) \to Y$.
\end{proof}

\begin{crl}
\label{SC and BSC}
Suppose that $k$ is a local field or a finite field endowed with the trivial valuation.
\begin{itemize}
\item[(i)] The space $\m{SC}_k(X)$ is homeomorphic to $\m{BSC}_k(X)$ under $X$.
\item[(ii)] The space $\m{BSC}_k(X)$ satisfies the extension property for a bounded continuous $k$-valued function on $X$.
\item[(iii)] The natural homomorphism $\m{C}(\m{BSC}_k(X),k) \to \m{C}_{\m{bd}}(X,k)$ is an isometric isomorphism.
\item[(iv)] The space $\m{BSC}_k(X)$ consists of $k$-rational points and the residue field of every maximal ideal of $\m{C}_{\m{bd}}(X,k)$ is $k$.
\end{itemize}
\end{crl}

We remark that (iv) is a partial generalisation of \cite{EM1} Theorem 7, which states that when $X$ is an ultrametric space and $k$ is locally compact, then the residue field of every maximal ideal of $\m{C}_{\m{bd}}(X,k)$ and the closed $k$-subalgebra of bounded uniformly continuous functions is $k$.

\begin{proof}
We deal only with (iv). We recall that for a Banach $k$-algebra $\A$, an $x \in \M_k(\A)$ is said to be a $k$-rational point if its support $\set{f \in A}{x(f) = 0}$ is a maximal ideal of $\A$ whose residue field is $k$. The isomorphism $\m{C}(\m{BSC}_k(X),k) \to \m{C}_{\m{bd}}(X,k)$ in (iii) gives an identification $\m{BSC}_k(X) = \M_k(\m{C}(\m{BSC}_k(X),k))$. The assertion immediately follows from a non-Archimedean generalisation of Stone--Weierstrass theorem (\cite{Ber1} 9.2.5.\ Theorem (i)) for $\m{C}(\m{BSC}_k(X),k)$.
\end{proof}

In particular, concerning Corollary \ref{SC and BSC} (iv), any point of $\m{BSC}_k(X)$ is peaked in the sense that the complete residue field is a peaked Banach $k$-algebra (\cite{Ber1} 5.2.1,\ Definition). A Banach $k$-algebra $\A$ is said to be {\it peaked} if for any extension $K/k$ of complete valuation fields, the norm on $\A \hat{\otimes}_k K$ is multiplicative. The notion of a peaked point is useful when we consider the topology-theoretical multiplication of points of analytic group. Corollary \ref{SC and BSC} (iv) does not hold when $k = \C_p$. Indeed, consider the rigid analytic disc $\m{D}^1(\C_p) \coloneqq \M_{\C_p}(\C_p \{ z \})$. It admits a natural embedding $\C_p^{\circ} \hookrightarrow \m{D}^1(\C_p)$ into a dense subset. The bounded $\C_p$-algebra homomorphism $\varphi \colon \C_p \{ z \} \to \m{C}_{\m{bd}}(\C_p^{\circ},\C_p)$ sending the variable $z$ to the coordinate function $z \colon \C_p^{\circ} \hookrightarrow \C_p$ induces a continuous map $\varphi^* \colon \m{BSC}_{\C_p}(\C_p^{\circ}) \to \m{D}^1(\C_p)$ under $\C_p^{\circ}$. Since $\m{BSC}_{\C_p}(\C_p^{\circ})$ and $\m{D}^1(\C_p)$ are compact Hausdorff spaces, the image of $\varphi^*$ contains the closure of the dense subset $\C_p^{\circ} \subset \m{D}^1(\C_p)$. Therefore $\varphi^*$ is surjective. Since $\C_p$ is not spherically complete, there is a $y \in \m{D}^1(\C_p)$ of type $4$. Take an $x \in \m{BSC}_{\C_p}(\C_p^{\circ})$ in $\varphi^{-1}(y)$. The induced bounded $\C_p$-algebra homomorphism $\varphi_x \colon \C_p \{ z \}/\m{supp}(y) \to \m{C}_{\m{bd}}(\C_p^{\circ},\C_p)/\m{supp}(x)$ gives an extension of fields transcendental over $\C_p$ because $y$ is of type $4$. Thus the point $x \in \m{BSC}_{\C_p}(\C_p^{\circ})$ is not $\C_p$-rational.

